Plug-and-Play Transformer Modules for Test-Time Adaptation

Parameter-efficient tuning (PET) methods such as LoRA, Adapter, and Visual Prompt Tuning (VPT) have found success in enabling adaptation to new domains by tuning small modules within a transformer model. However, the number of domains encountered during test time can be very large, and the data is usually unlabeled. Thus, adaptation to new domains is challenging; it is also impractical to generate customized tuned modules for each such domain. Toward addressing these challenges, this work introduces PLUTO: a Plug-and-pLay modUlar Test-time domain adaptatiOn strategy. We pre-train a large set of modules, each specialized for different source domains, effectively creating a ``module store''. Given a target domain with few-shot unlabeled data, we introduce an unsupervised test-time adaptation (TTA) method to (1) select a sparse subset of relevant modules from this store and (2) create a weighted combination of selected modules without tuning their weights. This plug-and-play nature enables us to harness multiple most-relevant source domains in a single inference call. Comprehensive evaluations demonstrate that PLUTO uniformly outperforms alternative TTA methods and that selecting $\leq$5 modules suffice to extract most of the benefit. At a high level, our method equips pre-trained transformers with the capability to dynamically adapt to new domains, motivating a new paradigm for efficient and scalable domain adaptation.

==> tables/dynamic/Forgetting_Cyclic.tex <==
\begin{table*}[t]
\centering
\caption{
\textbf{Comparing the issue of forgetting to the baselines on CIFAR-10}, this table shows that PLUTO displays significantly slower forgetting rates over an extended cycle of repetitive test distributions in comparison to the baseline methods. It's worth noting that the "online" methods, which rely on additional domain knowledge, serve as upper bounds for their respective continuous adaptation counterparts.}
\resizebox{1\textwidth}{!}{\begin{tabular}{c|ccccccccccccc}
\hline
\textbf{Time}      & \textbf{$t$}  & \textbf{}     & \textbf{}     & \textbf{}                          &               &               &               &                                    &               &               &               &                                    &               \\ \hline
Round              & 1             &               &               & \multicolumn{1}{c|}{}              & 3             &               &               & \multicolumn{1}{c|}{}              & 5             &               &               & \multicolumn{1}{c|}{}              & All           \\ \hline
Conditions         & Clean         & Snow          & Fog           & \multicolumn{1}{c|}{Frost}         & Clean         & Snow          & Fog           & \multicolumn{1}{c|}{Frost}         & Clean         & Snow          & Fog           & \multicolumn{1}{c|}{Frost}         & Avg           \\ \hline
TENT-Best-Online   & 89.9          & 87.7          & 87.6          & \multicolumn{1}{c|}{90.4}          & 89.9          & 87.7          & 87.6          & \multicolumn{1}{c|}{90.4}          & 89.9          & 87.7          & 87.6          & \multicolumn{1}{c|}{90.4}          & 88.9          \\
TENT-Ens-Online    & 94.1          & 91.1          & 93.8          & \multicolumn{1}{c|}{92.5}          & 94.1          & 91.1          & 93.8          & \multicolumn{1}{c|}{92.5}          & 94.1          & 91.1          & 93.8          & \multicolumn{1}{c|}{92.5}          & 92.9          \\
TENT-Ens-SA-Online & 94.3          & 91.4          & 94            & \multicolumn{1}{c|}{93.1}          & 94.3          & 91.4          & 94            & \multicolumn{1}{c|}{93.1}          & 94.3          & 91.4          & 94            & \multicolumn{1}{c|}{93.1}          & 93.2          \\
PLUTO-Online       & \textbf{95.1} & \textbf{93.3} & \textbf{94.4} & \multicolumn{1}{c|}{\textbf{94.4}} & \textbf{95.1} & \textbf{93.3} & \textbf{94.4} & \multicolumn{1}{c|}{\textbf{94.4}} & \textbf{95.1} & \textbf{93.3} & \textbf{94.4} & \multicolumn{1}{c|}{\textbf{94.4}} & \textbf{94.3} \\ \hline
TENT-Best          & 89.9          & 78.9          & 82.1          & \multicolumn{1}{c|}{70.2}          & 53.7          & 45.8          & 50.6          & \multicolumn{1}{c|}{47}            & 40.7          & 29.7          & 31.1          & \multicolumn{1}{c|}{27.4}          & 53.9          \\
TENT-Ens           & 94.1          & 85.2          & 83.1          & \multicolumn{1}{c|}{77.5}          & 61.8          & 54.4          & 52.3          & \multicolumn{1}{c|}{47.5}          & 35.2          & 30.4          & 30.8          & \multicolumn{1}{c|}{28.7}          & 56.7          \\
TENT-Ens-SA        & 94.3          & 88.2          & 83.7          & \multicolumn{1}{c|}{80.6}          & 66.7          & 57.5          & 59.7          & \multicolumn{1}{c|}{62.8}          & 57.4          & 40.6          & 30.8          & \multicolumn{1}{c|}{43.1}          & 63.7          \\
PLUTO              & \textbf{95.1} & \textbf{92.5} & \textbf{93.9} & \multicolumn{1}{c|}{\textbf{92.2}} & \textbf{89.1} & \textbf{92.6} & \textbf{89.5} & \multicolumn{1}{c|}{\textbf{88.6}} & \textbf{87.3} & \textbf{87.8} & \textbf{86.9} & \multicolumn{1}{c|}{\textbf{87.9}} & \textbf{90.3}
\label{table:forgetting_cyclic}
\end{tabular}}
\end{table*}

==> tables/stationary/ImageNetC_Few_shot.tex <==
\begin{table*}[t]

\centering
\caption{\textbf{Few-shot performance of \PLUTO.} On ImageNet-C (severity level=2) dataset, we train 15 modules for 15 domains. For the test-time adaptation performance evaluation, we pick 14 of them to adapt to the rest one. We randomly pick $U<B$ samples in the test batch to update module selector, make module selection, and LN tuning adaptation. We report the averaged accuracy over 15 target domains for different choice of $U$. $\mathcal{G}$ is pretrained on 15 source domains in a supervised manner.
}
\resizebox{\textwidth}{!}{\begin{tabular}{c c|c|c|c|c|c|c}
\hline
                          & Description                                                                    & $U=B=128$ & $U=64,B=128$ & $U=32,B=128$ & $U=16,B=128$ & $U=4,B=128$ & \makecell{$U=0$,\\Zero-shot}  \\ \hline
\multirow{4}{*}{Baseline} & Fully-finetune on $T_{target}$                                                     & 76.7    & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}       & \textcolor{lightgray}{$N/A$}  \\ \cline{2-8} 
                          & Supervised PET on $T_{target}$                                                     & 72.1    & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}       & \textcolor{lightgray}{$N/A$}  \\ \cline{2-8} 
                          & \makecell{Randomly select $M=5$ modules,
                          \\No adaptation} & \textcolor{lightgray}{$N/A$}     & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}        & \textcolor{lightgray}{$N/A$}       & 42.2 \\ \hline
\multirow{5}{*}{\PLUTO}    & \makecell{Supervised update to module selector $\mathcal{G}$ on $T_{target}$,\\Adaptation with $N=14$ modules} & 68.2    & 67.5       & 67.1       & 65.3       & 63.1      & \textcolor{lightgray}{$N/A$}  \\ \cline{2-8} 
                          & \makecell{Unlabeled update to module selector $\mathcal{G}$,\\Adaptation with $M=N=14$ modules selected} & 64.4    & 63.1       & 62.2       & 60.9       & 57.4      & 50.1 \\ \cline{2-8} 
                          & \makecell{Unlabeled update to module selector $\mathcal{G}$,\\Adaptation with M=5 modules selected}    & 63.7    & 62.2       & 61.2       & 59.4       & 56.3      & 47.3 \\ \hline
                          \label{table:fewshot}
\end{tabular}}
\end{table*}
